Model-Agnostic Few-Shot Open-Set Recognition

We tackle the Few-Shot Open-Set Recognition (FSOSR) problem, i.e. classifying instances among a set of classes for which we only have few labeled samples, while simultaneously detecting instances that do not belong to any known class. Departing from existing literature, we focus on developing model-agnostic inference methods that can be plugged into any existing model, regardless of its architecture or its training procedure. Through evaluating the embedding's quality of a variety of models, we quantify the intrinsic difficulty of model-agnostic FSOSR. Furthermore, a fair empirical evaluation suggests that the naive combination of a kNN detector and a prototypical classifier ranks before specialized or complex methods in the inductive setting of FSOSR. These observations motivated us to resort to transduction, as a popular and practical relaxation of standard few-shot learning problems. We introduce an Open Set Transductive Information Maximization method OSTIM, which hallucinates an outlier prototype while maximizing the mutual information between extracted features and assignments. Through extensive experiments spanning 5 datasets, we show that OSTIM surpasses both inductive and existing transductive methods in detecting open-set instances while competing with the strongest transductive methods in classifying closed-set instances. We further show that OSTIM's model agnosticity allows it to successfully leverage the strong expressive abilities of the latest architectures and training strategies without any hyperparameter modification, a promising sign that architectural advances to come will continue to positively impact OSTIM's performances.

==> checklist.tex <==
\section*{Checklist}


%%% BEGIN INSTRUCTIONS %%%
% The checklist follows the references.  Please
% read the checklist guidelines carefully for information on how to answer these
% questions.  For each question, change the default \answerTODO{} to \answerYes{},
% \answerNo{}, or \answerNA{}.  You are strongly encouraged to include a {\bf
% justification to your answer}, either by referencing the appropriate section of
% your paper or providing a brief inline description.  For example:
% \begin{itemize}
%   \item Did you include the license to the code and datasets? \answerNo{}
%   \item Did you include the license to the code and datasets? \answerNo{The code and the data are proprietary.}
%   \item Did you include the license to the code and datasets? \answerNA{}
% \end{itemize}
% Please do not modify the questions and only use the provided macros for your
% answers.  Note that the Checklist section does not count towards the page
% limit.  In your paper, please delete this instructions block and only keep the
% Checklist section heading above along with the questions/answers below.
%%% END INSTRUCTIONS %%%


\begin{enumerate}


\item For all authors...
\begin{enumerate}
  \item Do the main claims made in the abstract and introduction accurately reflect the paper's contributions and scope?
    \answerYes{}
  \item Did you describe the limitations of your work?
    \answerYes{See Section \ref{sec:discussions}}
  \item Did you discuss any potential negative societal impacts of your work?
    \answerNA{We didn't identify any potential negative societal impacts of our contributions.}
  \item Have you read the ethics review guidelines and ensured that your paper conforms to them?
    \answerYes{}
\end{enumerate}


\item If you are including theoretical results...
\begin{enumerate}
  \item Did you state the full set of assumptions of all theoretical results?
    \answerNA{}
        \item Did you include complete proofs of all theoretical results?
    \answerNA{}
\end{enumerate}


\item If you ran experiments...
\begin{enumerate}
  \item Did you include the code, data, and instructions needed to reproduce the main experimental results (either in the supplemental material or as a URL)?
    \answerYes{All instructions to reproduce results are provided in the README.md as part of the supplementary material.}
  \item Did you specify all the training details (e.g., data splits, hyperparameters, how they were chosen)?
    \answerYes{The hyper-parameter selection protocol is described in Section \ref{sec:experiments}. The exact list of hyperparameters tested for each method are contained in the .yaml config files, under the `configs/` in the code. Please refer to the README.md for exact instructions.}
        \item Did you report error bars (e.g., with respect to the random seed after running experiments multiple times)?
    \answerYes{Confidence intervals are showed in Table \ref{tab:benchmark_results_mini}.}
        \item Did you include the total amount of compute and the type of resources used (e.g., type of GPUs, internal cluster, or cloud provider)?
    \answerNA{As our method is inference-only, we didn't need to use GPUs to train a model. We used a single GPU for inference.}
\end{enumerate}


\item If you are using existing assets (e.g., code, data, models) or curating/releasing new assets...
\begin{enumerate}
  \item If your work uses existing assets, did you cite the creators?
    \answerYes{We cite all datasets and methods used in Sec. \ref{sec:experiments}. As for the models, we use pretrained checkpoints from \textsc{FEAT}'s repository and \textsc{TIMM} library, both of which we also cite in Sec. \ref{sec:experiments}.}
  \item Did you mention the license of the assets?
    \answerNA{}
  \item Did you include any new assets either in the supplemental material or as a URL?
    \answerYes{We include our code.}
  \item Did you discuss whether and how consent was obtained from people whose data you're using/curating?
    \answerNA{}
  \item Did you discuss whether the data you are using/curating contains personally identifiable information or offensive content?
    \answerNo{We exclusively used data that was previously used in peer-reviewed publications (see Section \ref{sec:experiments}).}
\end{enumerate}


\item If you used crowdsourcing or conducted research with human subjects...
\begin{enumerate}
  \item Did you include the full text of instructions given to participants and screenshots, if applicable?
    \answerNA{}
  \item Did you describe any potential participant risks, with links to Institutional Review Board (IRB) approvals, if applicable?
    \answerNA{}
  \item Did you include the estimated hourly wage paid to participants and the total amount spent on participant compensation?
    \answerNA{}
\end{enumerate}


\end{enumerate}

==> translations.tex <==
    \subsection{Formulation}

        Among the plethora of OOD detectors proposed in the litterature, we make the observation that the very basic $k$-NN detector, in coordination with standard feature normalizations is already a strong baseline for OOD, almost on par with state-of-the-art meta baselines recently proposed. Fueled by such empirical observations, we further investigate such baseline, and state the problem as follows. Given trained feature extractor $\phi: \mathcal{X} \rightarrow \mathcal{Z}$, and is given a task $\{\support, \query \}$, can one learn a simple feature transformation $\psi: \mathcal{Z} \rightarrow \mathcal{Z}$ such that a simple $k$-NN detector applied on top of $\{\psi(\support), \psi(\query)\}$ achieves high OOD detection performance ? Formally, one seeks to make outlier points as dissimilar from inliers as possible. One may achieve that goal by minimizing the following loss:

        \begin{align} \label{eq:ideal_objective}
            \min_{\psi} ~ \mathcal{L}(\psi; \support, \zseen, \zunseen) =& \sum_{\zbf_q \in \query} \mathbbm{1}[\zbf_q \in \zunseen] \sum_{\zbf_s \in \support} w_{s,q} ~ \dotprod{\psi(\zbf_q)}{\psi(\zbf_s)} \\
                &- \sum_{\zbf_s \in \support} \sum_{\zbf_{s'} \in \support} \dotprod{\psi(\zbf_s)}{\psi(\zbf_{s'})}
            % - \sum_{z: y \in \seen} \phi(z)^T (\frac{1}{|\support|} \sum_{s \in \support} \phi(s)) \\
             % &= \sum_{z: y \in \unseen} \phi(z)^T \mubf_{sup}  - \sum_{z: y \in \seen} \phi(z)^T \mubf_{sup} \\
        \end{align}

        where $w_{s,q}$ equals 1 if $\psi(\zbf_s)$ belongs to the $k$-nearest neighbors of $\psi(\zbf_q)$, 0 otherwise. An obvious problem with Eq. \eqref{eq:ideal_objective} is that we do not have access to the ground truth $\mathbbm{1}[\zbf_q \in \zunseen]$. In order to address this issue, we simply introduce soft assignment variables $\{s_{q}\}_{q=1}^{|\mathcal{Q}|} \in [0,1]$ that are optimized alongside the parameters of $\psi$, and aims to reflect the likelihood of some query point to be an outlier. In order to penalize overly confident, potentially overfitted, solutions, e.g. $s_q=0$ or $s_q=1$, we use a standard negentropy regularization term. The resulting objective functions reads:

        \begin{align} \label{eq:approx_objective}
            \min_{\psi} ~ \mathcal{L}(\psi, \sbf; \support, \zseen, \zunseen) =& \quad \sum_{\zbf_q \in \query} s_q ~  \sum_{\zbf_s \in \zseen} w_{s,q} ~ \dotprod{\psi(\zbf_q)}{\psi(\zbf_s)} - \frac{1}{\lambda} \sum_q H_{2}(s_q) \\ &- \sum_{\zbf_q \in \support} \sum_{\zbf_s \in \support} w_{s,q} ~ \dotprod{\psi(\zbf_q)}{\psi(\zbf_s)} \\
            \text{subject to} ~ & \quad s_q \in [0, 1]
            % - \sum_{z: y \in \seen} \phi(z)^T (\frac{1}{|\support|} \sum_{s \in \support} \phi(s)) \\
             % &= \sum_{z: y \in \unseen} \phi(z)^T \mubf_{sup}  - \sum_{z: y \in \seen} \phi(z)^T \mubf_{sup} \\
        \end{align}
        where $H_{2}(s_q) = - s_q \log(s_q)  - (1-s_q) \log(1 - s_q)$ is the binary entropy and encourages smooth $s_q$, and $\lambda$ is a hyper-parameter. 

        \begin{lemma} \label{lemma:optimal_s}
            For a fixed $\psi$ transformation, Problem \eqref{eq:approx_objective} can be globally minimized. The optimal solution $\sbf^*$ is then given by:
            \begin{align} \label{eq:optimal_s}
                s_q^* = \sigma (-\lambda \dotprod{\psi(\zbf_q)}{\sum_{\zbf \in \zseen} w_{q,s} \psi(\zbf_s)})
            \end{align}
        where $\sigma$ stands for the sigmoid function.
        \end{lemma}

        \begin{proof}
            The first part of the objective function is linear in $\sbf$, while the negentropy is strictly convex. Therefore, the addition of the functions is a strictly convex objective. Taking the gradients of $\mathcal{L}$ w.r.t $\sbf$ yields:
            \begin{align}
                \nabla_{s_q}~\mathcal{L} =& \dotprod{\psi(\zbf_q)}{\sum_{\zbf \in \zseen} w_{q,s} \psi(\zbf_s)} + \frac{1}{\lambda} (\log(s_q) + 1 - (\log(1 - s_q) + 1)) \\
                 =& \dotprod{\psi(\zbf_q)}{\sum_{\zbf \in \zseen} w_{q,s} \psi(\zbf_s)} + \frac{1}{\lambda} \log \left(\frac{s_q}{1 - s_q} \right)
            \end{align}
            Finding stationnary points satisfying $\nabla_{s_q}~\mathcal{L}(s_q^*) = 0$:
            \begin{align}
                & \log\left(\frac{s_q^*}{1-s_q^*}\right) = \sigma^{-1}(s_q^*) = \left(-\lambda \dotprod{\psi(\zbf_q)}{\sum_{\zbf \in \zseen} w_{q,s} \psi(\zbf_s)} \right) \\
                \iff \quad & s_q^* = \sigma\left(-\lambda \dotprod{\psi(\zbf_q)}{\sum_{\zbf \in \zseen} w_{q,s} \psi(\zbf_s)} \right)
            \end{align}
            Note that this global solution automatically satisfies the constraint $s_q^* \in [0,1]$, which a posteriori justifies not explictly handling such constraint.

        \end{proof}

        \paragraph{Choice of $\psi$} 
            
            Several works \cite{kriegel2008angle} from the standard OOD detection litterature have noticed that $\ell_2$ normalization was effective in boosting OOD detectors. However, a simple geometric intuition (ADD DRAWING HERE) shows that mere L2 normalization is not ideal. In particular, it was shown in standard classification \cite{wang2019simpleshot} that preceding $\ell_2$ normalization by a simple translation:
            \begin{align}
                \psi(\zbf; \mubf) = \frac{\zbf - \mubf}{\norm{\zbf - \mubf}}
            \end{align}
            could help improve results. We adopt such transformation, as it complies with our target to limit the amount of learnable parameters.

        \paragraph{Optimization}

            At inference, we propose to learn the parameters $\{\sbf, \mubf \}$ in an alternate fashion. In particular, 

            \begin{enumerate}
                \item Update $\mubf$ with a gradient step
                \item Update $\sbf$ using Eq. \eqref{eq:optimal_s}
            \end{enumerate}
                        
        %     \begin{lemma}\label{lemma:supporting_hyperplane}
        %         Let A be a convex set, and let $\mubf \notin A$. Let us also consider $\zbf^{*} = \text{proj}_{A}(\mubf) = \argmin_{\zbf \in A} \norm{\zbf - \mubf}$. Then $H(\pbf, b) = \{ \zbf: \dotprod{\pbf}{\zbf} \geq b \}$, with $\pbf=\zbf^{*} - \mubf$ and $b=\dotprod{\pbf}{\zbf^{*}}$, is a supporting hyperplane of $A$ and separates $\mubf$ from A.
        %     \end{lemma}
        
        % \begin{proof}
        
        %     We first need to show that $\dotprod{\pbf}{\mubf} \leq b$. Indeed, 
        %     \begin{align}
        %         \dotprod{\pbf}{\mubf} - b = \dotprod{\zbf^{*} - \mubf}{\mubf - \zbf^{*}} =  - \norm{\mubf - \zbf^{*}}^2 \leq 0
        %     \end{align}
            
        %     Now, let us consider $\zbf \in A$ and let's show that $\dotprod{\pbf}{\zbf} \geq b$. Let us prove this by contradiction. Assume that there exists $\zbf \in A$ such that $\dotprod{\pbf}{\zbf - \zbf^*} < 0$. Then, consider points lying on the line between $\zbf$ and $\zbf^{*}$:
        %     \begin{align}
        %         \zbf^{\lambda} = \lambda \zbf + (1-\lambda) \zbf^{*}
        %     \end{align}
        %     Note that $\zbf^{\lambda} \in A$ by convexity of $A$. We can show that there exists an interval in which $\norm{\zbf^{\lambda} - \mubf}^2 < \norm{\zbf^{*} - \mubf}^2 = \norm{\pbf}^2$ which contradicts that $\zbf^{*}$ is the projection of $\mubf$ on A. Indeed:
        %     \begin{align}
        %         \norm{\zbf^{\lambda} - \mubf}^2 - \norm{\pbf}^2 &= \norm{\pbf + \lambda.(\zbf - \zbf^{*})}^2 - \norm{\pbf}^2\\
        %         &= \lambda~ (2~\dotprod{\pbf}{\zbf - \zbf^{*}} + \lambda \norm{\zbf - \zbf^*}^2) \
        %     \end{align}
        %     Therefore, for $\lambda \in \displaystyle{]0, \frac{- 2~\dotprod{\pbf}{\zbf - \zbf^{*}}}{\norm{\zbf - \zbf^*}^2} [}$~, we have $\norm{\zbf^{\lambda} - \mubf}^2 - \norm{\pbf}^2 < 0$, which is a contradiction.

        % \end{proof}

        % \begin{lemma}\label{lemma:outside_convex_hull}
        %     For $\mubf$ outside the convex hull of the task, the loss $\mathcal{L}(\mubf)$ can never reach the minimum value of -1. Formally, $\forall \mubf \notin \convhull{\support, ~ \zunseen}, ~ \mathcal{L}(\mubf) >  \mathcal{L}_{min}=-1$.
        % \end{lemma}

        \begin{proof}
            For notation simplicity, let us denote $A=\convhull{\support, ~ \zunseen}$. 

            Let us consider $\mubf \notin A$. Then, we know by Lemma \ref{lemma:supporting_hyperplane} that $H(\pbf, b) = \{ \zbf: \dotprod{\pbf}{\zbf} \geq b \}$, with $\pbf=\zbf^{*} - \mubf$,  $b=\dotprod{\pbf}{\zbf^{*}}$ and $\zbf^{*} = \text{proj}_{A}(\mubf)$ is a supporting hyperplane of $A$.

            Now, we can prove that $\forall ~ (\zbf_i, \zbf_j) \in A, \dotprod{\zbf_i - \mubf}{\zbf_j - \mubf} > 0$:
            \begin{align}
                \dotprod{\zbf_i - \mubf}{\zbf_j - \mubf} &= \dotprod{\zbf_i - \zbf^{*} + \zbf^* - \mubf}{\zbf_j - \zbf^{*} + \zbf^* - \mubf} \\
                &= \dotprod{\zbf_i - \zbf^{*} + \pbf}{\zbf_j - \zbf^{*} + \pbf} \\
                &= \underbrace{\dotprod{\zbf_i - \zbf^{*}}{\zbf_j - \zbf^{*}}}_{\geq - \norm{\zbf_i - \zbf^{*}}\norm{\zbf_j - \zbf^{*}} } + \underbrace{\dotprod{\zbf_i - \zbf^{*}}{\pbf}}_{\geq 0 ~ \text{by def of ~} H} + \underbrace{\dotprod{\pbf}{\zbf_j - \zbf^{*}}}_{\geq 0 ~ \text{by def of ~} H} + \underbrace{\norm{\pbf}^2}_{>0} \\
                &> - \norm{\zbf_i - \zbf^{*}}\norm{\zbf_j - \zbf^{*}}
            \end{align}
            Therefore
            \begin{align}
                \dotprod{\phi_{\mubf}(\zbf_i)}{\phi_{\mubf}(\zbf_i)} > - \frac{\norm{\zbf_i - \zbf^{*}}\norm{\zbf_j - \zbf^{*}}}{\norm{\zbf_i - \mubf}\norm{\zbf_j - \mubf}} \geq -1
            \end{align}
            Which directly implies that:
            \begin{align}
                \mathcal{L}(\mubf) = \frac{1}{|\zunseen|~|\support|} \sum_{\zbf_u \in \zunseen} \sum_{\zbf_s \in \support} \dotprod{\phi_{\mubf}(\zbf_u)}{\phi_{\mubf}(\zbf_s))} > -1
            \end{align}
        \end{proof}
